Adventures in Demand Analysis Using AI

This paper advances empirical demand analysis by integrating multimodal product representations derived from artificial intelligence (AI). Using a detailed dataset of toy cars on textit{Amazon.com}, we combine text descriptions, images, and tabular covariates to represent each product using transformer-based embedding models. These embeddings capture nuanced attributes, such as quality, branding, and visual characteristics, that traditional methods often struggle to summarize. Moreover, we fine-tune these embeddings for causal inference tasks. We show that the resulting embeddings substantially improve the predictive accuracy of sales ranks and prices and that they lead to more credible causal estimates of price elasticity. Notably, we uncover strong heterogeneity in price elasticity driven by these product-specific features. Our findings illustrate that AI-driven representations can enrich and modernize empirical demand analysis. The insights generated may also prove valuable for applied causal inference more broadly.

==> JASA_Buybox_Version/Absract.tex <==
\noindent This paper advances empirical demand analysis by integrating multimodal product representations derived from artificial intelligence (AI). 
%
Using a detailed dataset of toy cars on \textit{Amazon.com}, we combine text descriptions, images, and tabular covariates to represent each product using transformer-based embedding models. 
%
These embeddings capture nuanced attributes, such as quality, branding, and visual characteristics, that traditional methods often struggle to summarize. 
%
Moreover, we fine-tune these embeddings for causal inference tasks. 
%
We show that the resulting embeddings substantially improve the predictive accuracy of sales ranks and prices and that they lead to more credible causal estimates of price elasticity. 
%
Notably, we uncover strong heterogeneity in price elasticity driven by these product-specific features. 
%
Our findings illustrate that AI-driven representations can enrich and modernize empirical demand analysis. 
%
The insights generated may also prove valuable for applied causal inference more broadly.

\smallskip

\noindent%
{\it Keywords:} Causal Inference; Deep Embeddings; Causal Fine-Tuning; Text; Images; Panel Data; Debiased Machine Learning; Demand Analysis; Foundation Models.
\vfill
